Frontiers in Mortar Methods for Isogeometric Analysis

Complex geometries as common in industrial applications consist of multiple patches, if spline based parametrizations are used. The requirements for the generation of analysis-suitable models are increasing dramatically since isogeometric analysis is directly based on the spline parametrization and nowadays used for the calculation of higher-order partial differential equations. The computational, or more general, the engineering analysis necessitates suitable coupling techniques between the different patches. Mortar methods have been successfully applied for coupling of patches and for contact mechanics in recent years to resolve the arising issues within the interface. We present here current achievements in the design of mortar technologies in isogeometric analysis within the Priority Program SPP 1748, Reliable Simulation Techniques in Solid Mechanics. Development of Non-standard Discretisation Methods, Mechanical and Mathematical Analysis.

==> chapters/contact3.tex <==
\subsection{Hierarchical NURBS and fracture contact mechanics}

In this last subsection concerning mortar contact methods, two central goals are taken into account: Hierarchical refinement schemes to deal with local refinements in the contact area and fracture for high-velocity impact simulations. The formulation presented here are taken from \cite{hesch2016a}, where an in-depth investigation is shown in detail. 

To start with local refinement schemes, we note that classical refinement procedures rely on the subdivision of elements. This is not an applicable procedure for higher-order problems, since the classical approaches do not conserve the required higher continuity. To circumvent this issue, we focus on a subdivision of the basis functions themselves. This allows us to maintain the required continuity by replacing the underlying B-splines using a linear combination of splines via
\begin{equation}\label{eq:refinement}
 B^{k,A} = B^{k,\vec{i}}_{\vec{p}}(\vec{\xi}) =
 \sum\limits_{\vec{j}=\vec{0}}^{\vec{p}+\vec{1}}\prod\limits_{l = 1}^{d}2^{-p_l}\,\binom{p_{l}+1}{j_l}\,N_{i_l,p_l}\,(2\,\xi^l-j_l\,h_l-\xi_{i_l}^l),
\end{equation}
where \(h_l\) refers to the coarse level element length in the parameter space. An example for a two-dimensional example is shown in Figure \ref{fig:sub_2D}.
\begin{figure}
\begin{center}
\includegraphics[width=0.85\textwidth]{pictures/sub_2Dp}
\caption{Subdivision of 2D quadratic and cubic B-splines.}\label{fig:sub_2D}
\end{center}
\end{figure}
Since the refined level consists of copied and scaled versions of the original B-spline, further local refinements can be applied level by level. The extension of B-splines to NURBS reads 
\begin{equation}\label{eq:refNURBS}
R^{k,A} = R^{k,\vec{i}}_{\vec{p}}(\vec{\xi}) = \frac{\sum\limits_{\vec{j}=\vec{0}}^{\vec{p}+\vec{1}}S_{\vec{i},\vec{j}}\,B^{k+1,2\vec{i-1}+\vec{j}}_{\vec{p}}(\vec{\xi})\,w^{k+1}_{2\vec{i}-\vec{1}+\vec{j}}}{\sum\limits_{\vec{i}}\sum\limits_{\vec{j}=\vec{0}}^{\vec{p}+\vec{1}}S_{\vec{i},\vec{j}}\,B^{k+1,2\vec{i-1}+\vec{j}}_{\vec{p}}(\vec{\xi})\,w^{k+1}_{2\vec{i}-\vec{1}+\vec{j}}},
\end{equation}
where we have introduced a subdivision matrix, such that
\begin{equation}
B^{k,\vec{i}}_{\vec{p}}(\vec{\xi}) = \sum\limits_{\vec{j}=\vec{0}}^{\vec{p}+\vec{1}}S_{\vec{i},\vec{j}}\,B^{k+1,2\vec{i-1}+\vec{j}}_{\vec{p}}(\vec{\xi}),\quad\text{and}\quad
\vec{q}_A^{k+1} = \vec{S}_A^T\,\vec{q}_A^{k}.
\end{equation}
Note that (\ref{eq:refinement}) is only valid for uniform knot vectors and has to be modified for non-uniform knot vectors. For further details, e.g. for the case of repeated knots, details on the construction of the subdivision matrix and its application to control points of NURBS instead of B-spline basis functions as well as the numerical evaluation of the finite elements, see Hesch et al. \cite{hesch2016b}.

\begin{figure}[t]
\begin{center}
\footnotesize
\begin{tabular}{cc}
\includegraphics[width=0.57\textwidth]{pictures/HNPF_ref2}\hspace{1mm}
\includegraphics[width=0.4\textwidth]{pictures/loadDisPlate.eps}
\end{tabular}
\end{center}
\caption{\textbf{Bending contact fracture problem.} Reference configuration (left) and load-displacement curve (right).}
\label{fig:cpMod4}
\end{figure}

Within a Lagrangian formulation as introduced before in the context of finite deformation elasticity, we describe a phase-field by an order parameter $\s(\vec{X},t):\mathcal{B}_{0}\times\mathcal{I}\rightarrow\mathbb{R},\quad\s\in[0,1]$, and approximate the critical fracture energy as
\begin{equation}
\int\limits_{\Gamma_0^{cr}}g_c\d\Gamma \approx \int\limits_{\Omega_0}g_c\,\gamma(\s)\d V.
\end{equation}
Therefore,we apply a fourth-order approach for the crack-density function $\gamma(\s) = 1/(4\, l)\,\s^2 + l/2\,\nabla(\s)\cdot\nabla(\s) + l^3/4\,\Delta^2(\s)$, which requires at least $C^1$ continuous shape functions. Following central ideas of gradient plasticity, we split the deformation gradient into a fracture sensitive and an insensitive part via an eigenvalue decomposition, such that
\begin{equation}
\tilde{\vec{F}} = \sum\limits_{a}(\lambda_a^+)^{(1-\s)}\,(\lambda_a^-)\,\vec{n}_a\otimes\vec{N}_a,
\end{equation}
where \(\vec{n}_a\) and \(\vec{N}_a\) denote the principal directions of the left and right stretch tensors. Moreover, \(\lambda_a\) are  principal stretches, decomposed into tensile and compressive components via \(\lambda_a^{\pm} = [(\lambda_a-1)\pm |\lambda_a-1|]/2+1\). This approach can be applied in a straight-forward manner to porous ductile thermomechanical fracture, as shown in \cite{hesch2019c}, where we have introduced a triple split of the deformation gradient, to consider the elastic, plastic and fracture parts. The mortar contact algorithm can now be adapted to the mechanical field, as the fracture field automatically reduces the stress within the contact area, if fracture takes place. The hierarchically refined areas can be applied to the mortar segmentation procedure using the geometrical information of the finest level. Note that the book keeping between the segments and the partially new generated nodes and the corresponding degrees of freedom is challenging.

As prototypical example to demonstrate the capabilities of the phase-field approach within a contact situation with hierarchical refinements, we introduce a plate as shown in Figure \ref{fig:cpMod4} left. The plate  is clamped and locally refined using a three-level hierarchical refinement on the right hand side. A further one-level refinement is applied to the plate as well as to the block within the expected contact area, such that in total 12948 elements with overall 72912 degrees of freedom are used. Note that a globally refined plate would require more than three million degrees of freedom without improvements on the accuracy of the areas of interest. The upper boundary of the block is moved downwards, until the plate is ripped out of the bearing, as can be seen in Figure \ref{fig:bendingContactFractureResults}. The corresponding load-displacement curve is shown in Figure \ref{fig:cpMod4}, right.

\begin{figure}[t]
\begin{center}
\begin{tabular}{cc}
\includegraphics[width=0.49\textwidth]{pictures/HNURBSphaseFieldStaticContactC3t10bPhasePaperColorbar582} &
\includegraphics[width=0.49\textwidth]{pictures/HNURBSphaseFieldStaticContactC3t10bStressPaperColorbar582}
\end{tabular}
\end{center}
\caption{\textbf{Bending contact fracture problem.} Phase-field after 582 steps (left) and \(\sigma_{22}\) stress distribution (right).}
\label{fig:bendingContactFractureResults}
\end{figure}


==> chapters/onethreedim.tex <==
%\todoB{Ustim: this is the section where you should add the text on the 1D-3D coupling}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\X}{\vec{X}}
\newcommand{\x}{\vec{x}}
\newcommand{\y}{\vec{y}}
\newcommand{\z}{\vec{z}}
\newcommand{\Id}{\operatorname*{Id}}
\newcommand{\sign}{\operatorname*{sign}}
%\newcommand{\op}[1]{\operatorname*{#1}}
\newcommand{\eps}{\varepsilon}
\newcommand{\J}{\mathcal{J}}
\newcommand{\dev}[1]{\text{dev}\left[#1\right]}
\newcommand{\norm}[1]{\lVert #1 \rVert}
\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\dt}{\Delta t}
\newcommand{\dx}{\Delta x}
\newcommand{\sgn}[1]{\ \text{sgn}\left(#1\right) }
\newcommand{\sca}[2]{\langle #1, \; #2 \rangle}
\newcommand{\frc}[2]{{\textstyle\frac{#1}{#2}}}
\newcommand{\minus}{\scalebox{0.7}[1.0]{\( - \)}}
\newcommand{\inv}{^{\scalebox{0.7}[1.0]{\( - \)}1}}%{^{-1}}
\newcommand{\tp}{^\intercal}
\newcommand{\tpc}{^*}
\renewcommand{\exp}[1]{e^{#1}}
\newcommand{\Exp}[1]{\operatorname*{Exp}\left(#1\right)}
%\renewcommand{\i}{\mathrm{i}}
\renewcommand{\d}{\operatorname{d}\!}
\newcommand{\tr}{\operatorname{tr}}
\renewcommand{\Re}{\mathfrak{Re}}
\renewcommand{\Im}{\mathfrak{Im}}
\newcommand{\B}{\lbrace -1, 1\rbrace}
\newcommand{\Ind}{\mathbbm{1}}
\renewcommand{\O}{\mathcal{O}}

% vectors and matrices
%\newcommand{\mat}[1]{\begin{bmatrix} #1 \end{bmatrix}}
\newcommand{\diag}{\operatorname{diag}}
\renewcommand{\vec}[1]{\pmb{#1}}
\newcommand{\vct}[1]{\vec{#1}}
\newcommand{\ten}[1]{\pmb{#1}}
\newcommand{\tns}[1]{\ten{#1}}
\newcommand{\tnsfour}[1]{\pmb{#1}}

% parantheses
\newcommand{\bbc}[1]{\left( #1 \right)}
\newcommand{\rbc}[1]{\left[ #1 \right]}

% differentiation
\newcommand{\drv}[2]{\frac{\partial #1}{\partial #2}} %{\partial_{#1} #2}
%\newcommand{\D}[2]{\partial_{#1} #2}
\renewcommand{\div}{\nabla\cdot}
%\newcommand{\grad}{\nabla}
\newcommand{\gradS}{\nabla\!_s}
\newcommand{\Jac}[2][]{ \operatorname*{D_{#1}}\! #2  }
\newcommand{\Hess}[1]{ D^2#1  }



% Sets
\newcommand{\Z}{\mathbb{Z}} % integer
\newcommand{\R}{\mathbb{R}} % real
\newcommand{\C}{\mathbb{C}} % complex
\newcommand{\N}{\mathbb{N}} % natural

% Matrix groups
\newcommand{\SymM}[1][3]{\op{S}^{#1}} % Symmetric matrices
\newcommand{\PSD}[1][3]{\SymM[#1]_+} % Symmetric positive semi-definite matrices
\newcommand{\PD}[1][3]{\SymM[#1]_{++}}  % Symmetric positive definite matrices
\newcommand{\SO}[1]{\operatorname{SO}_{#1}}  % Symmetric positive definite matrices

% Spaces
\newcommand{\HS}{\mathcal{H}} % Hilbert space
\newcommand{\K}{\mathcal{K}} % Krylov subspace
\renewcommand{\L}[1]{\op{L}^{\!#1}} % Lesbegues space
\newcommand{\W}[2]{\op{W}^{#1,#2}} % Sobolev space
\renewcommand{\H}[1]{\op{H}^{#1}} % Sobolev space
\newcommand{\Cn}[1]{\op{C}^{#1}} % Sobolev space
%\newcommand{\M}{\mathbb{M}} % Space of matrices
\newcommand{\vspan}{\op{span}} % convex hull (span)



% Coupling
\newcommand{\fib}[1]{\tilde{#1}}
\newcommand{\mtx}[1]{#1}
\newcommand{\axl}{\operatorname{axl}}
\newcommand{\Area}{A}
\newcommand{\Circ}{C}
\newcommand{\stiffnessC}{\ten{K}\!_1}
\newcommand{\stiffnessD}{\ten{K}\!_2}

\newcommand{\TrialSpace}{V^h}
\newcommand{\TestSpace}{\hat{V}^h}
\newcommand{\CollocSet}{\mathcal{S}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Let us consider a Lipschitz convex bounded domain~$\Omega\subset\R^3$, such that $\Omega = \Omega_{M}\cup\Omega_{F}$, where subdomains~$\Omega_{M}$ and $\Omega_{F}\subset\R^3$ correspond respectively to the material matrix and the fiber introduced in the matrix.
Let $\Gamma$ be the fiber/matrix interface, and $\partial\Omega_{N}$ be a part of the boundary~$\partial\Omega$ associated to Neumann boundary conditions.
The matrix and the fiber are presented respectively as Cauchy and Cosserat continua.
The displacement field is
\begin{equation}\label{key}
\x_{glo}(\X) =
\begin{cases}
\mtx{\x}(\X), & \text{ in } \Omega_{M}, \\
\fib{\x}(\X), & \text{ in } \Omega_{F}, \\
\end{cases}
\end{equation}
where $\mtx{\x}(\X)$ and $\fib{\x}(\X)$ denote deformation fields of matrix and fiber respectively.
Besides, $\fib{\ten{R}}(\X)$, $\X\in\Omega_{F}$, is orthogonal matrix of directors of the fiber. 
The total energy of the matrix/fiber system is
\begin{equation}\label{eq:Total_Energy}
%	W = \Pi_{M} + \Pi_{F} + \Pi_{interact} + \Pi_{ext},
\Pi = \Pi_{M} + \Pi_{F} + \Pi_{C},
\end{equation}
where $\Pi_{M}$ and $\Pi_{F}$ stand for the internal energy of the matrix and the fiber respectively, and $\Pi_{C}$ is the coupling term:
\begin{align}\label{key}
\Pi_{M} &= \int\limits_{\Omega_{M}} \Psi_{M} \d V
+
\int\limits_{\Omega_{M}} \vec{f}_{vol}\cdot\mtx{\vec{u}} \d V
+
\int\limits_{\partial\Omega_{N}} \vec{t}_{ext}\cdot\mtx{\vec{u}} \d V
, \\
\Pi_{F} &= \int\limits_{\Omega_{F}} \Psi_{F} \d V
+
\int\limits_{\Omega_{F}} \vec{f}_{vol}\cdot\fib{\vec{u}} \d V
, \\
\Pi_{C} &= \!\!\!\! \int\limits_{\Omega_{M}\cap\Omega_{F}}\!\!\!\!  \left(\mtx{\x}-\fib{\x}\right)\cdot\vec{\mu}\d V
- \!\!\!\! \int\limits_{\Omega_{M}\cap\Omega_{F}}\!\!\!\!  \frac{\alpha}{2}\,\vec{\mu}^2\d V
, \label{eq:fib:FreeEnergy}
\end{align}
where $\Psi_{M}$ and $\Psi_{F}$ denote internal free energy densities of the matrix and the fiber respectively,
%where $\mtx{\x}$ and $\fib{\x}$ denote displacement fields of matrix and fiber respectively, and $\fib{\ten{R}}$ is the directors matrix of the fiber.
%where $\ten{\eps}_{F} = \ten{\eps}_{F}(\nabla\fib{\x}, \fib{\ten{R}})$ is the Green--Lagrange strain tensor and $\ten{\kappa}_{F} = \ten{\kappa}_{F}(\nabla\fib{\x}, \fib{\ten{R}})$ is the curvature tensor, $\ten{C}$ and $\ten{D}$ are the corresponding stiffness higher order tensors.
%The fiber is presented as Cosserat media described by the displacement~$\fib{\x}$ and rotation tensor~$\fib{\ten{R}}$.
%Above, $\Pi_{interact}$ is the work of matrix/fiber interaction forces:
%\begin{align}\label{key}
%	\Pi_{interact} &= \int\limits_{\Omega_{M}\cap\Omega_{F}} \!\!\!\!\vec{t}_{int} \cdot(\mtx{\x}-\fib{\x})\d V,\\
%	\Pi_{ext} &= 
%	\int\limits_{\Omega_{M}\cup\Omega_{F}} \!\!\!\!\vec{f}_{vol}\cdot\vec{u} \d V
%	+
%	\int\limits_{\partial\Omega_{N}} \vec{t}_{ext}\cdot\vec{u} \d V,
%\end{align}
%where 
%$\rho_{M}$ and $\rho_{F}$ stand for the corresponding mass densities,
$\mtx{\vec{u}} = \mtx{\x}-\X$ and $\fib{\vec{u}} = \fib{\x}-\X$ are the displacement fields of the matrix and the fiber respectively,
$\vec{f}_{vol}$ and $\vec{t}_{ext}$ are respectively volumetric force density and external load applied on~$\partial\Omega_{N}$, 
and $\vec{\mu}$ is a Lagrange multiplier associated to the surface load on the matrix/fiber interface.
The coupling term~$\Pi_{C}$ in this form defines the fiber/matrix interaction of spring type:
the coefficient~$\alpha\ge0$ corresponds to the inverse spring stiffness.
In what follows we are going to consider the case~$\alpha=0$ (infinite stiffness), which corresponds to displacement continuity constraint on the interface.
%and $\vec{t}_{int}$ is the surface load on the matrix/fiber interface.
%and is also unknown, along with displacement field and the fiber directors.
%The form of the interface load~$\vec{t}_{int}$ is defined by the type of matrix/fiber coupling.
%For example, in case of soft coupling of spring type it writes as $\vec{t}_{int} = k\cdot(\mtx{\x}-\fib{\x})$, with $k$ being the stiffness.
%In what follows, we consider hard coupling implying displacement continuity constraints: $k\to\infty$, $\abs{\vec{t}_{int}}<\infty$, so that $\vec{t}_{int}$ plays role of Lagrange multiplier.
%The form of such multiplier also defines type of constraint.
%For example, the interface load of the form $\vec{t}_{int} = \alpha\cdot\vec{n}$, with a scalar Lagrange multiplier~$\alpha$ and $\vec{n}$ being a normal to the interface, corresponds to a non-penetration constraint.
%%and $\vec{t}_{int}$ is the interaction force density between matrix and fiber surfaces.

Thus, we have a saddle point optimization problem to solve:
\begin{equation}\label{key}
\inf\limits_{\x_{glo},\fib{\ten{R}}} \; \sup\limits_{\vec{\mu}} \; \Pi(\x_{glo},\fib{\ten{R}},\vec{\mu}).
\end{equation}
The corresponding Euler-Lagrange equation writes
\begin{multline}\label{eq:VariationalForm}
\int\limits_{\Omega_{M}} \drv{\Psi_{M}}{\mtx{\ten{F}}}:\ten{\delta \mtx{F}} \d V
+
\int\limits_{\Omega_{F}} \drv{\Psi_{F}}{\fib{\ten{F}}}:\ten{\delta\fib{F}} \d V
%+
%\int\limits_{\Omega_{F}} \ten{G}_{F}:\ten{\delta\fib{R}} \d V
%	+
%	\int\limits_{\Omega_{F}} \left(\ten{\eps}_{F}:\ten{C}:\ten{\delta\eps}_{F} + 	\ten{\kappa}_{F}:\ten{D}:\ten{\delta\kappa}_{F}\right) \d V
+\\
+
\!\!\!\!\int\limits_{\Omega_{M}\cap\Omega_{F}} \!\!\!\!\vec{\mu} \cdot(\vec{\delta\mtx{x}}-\vec{\delta\fib{x}})\d S
+
\!\!\!\!\int\limits_{\Omega_{M}\cap\Omega_{F}} \!\!\!\!\vec{\delta\mu} \cdot(\mtx{\x}-\fib{\x})\d S
%	+
%	\!\!\!\!\int\limits_{\Omega_{M}\cap\Omega_{F}} \!\!\!\!\vec{\mu} \cdot(\vec{\delta u}_{M}-\vec{\delta\fib{\varphi}})\d V
%	+
%	\!\!\!\!\int\limits_{\Omega_{M}\cap\Omega_{F}} \!\!\!\!\vec{\delta f}_{interact} \cdot(\mtx{\x}-\fib{\x})\d V
+ \\
+
\int\limits_{\Omega} \vec{f}_{vol}\cdot\vec{\delta x}_{glo} \d V
+
\int\limits_{\partial\Omega_{N}} \vec{t}_{ext}\cdot\vec{\delta x}_{glo} \d S
= 0.
\end{multline}
%where $\ten{P}_M$ and $\ten{P}_{F}$ are the $1$st Piola-Kirchhoff stress tensors of the matrix and the fiber respectively, and $\ten{G}_{F}$ is \rev{(What is $\ten{G}_{F}$ ??)}.
%, and $\ten{F}=\nabla\vec{u}$ is the deformation gradient.
Without loss of generality, we assume $\vec{f}_{vol}=0$ in what follows.

\subsection{Thin rigid fiber model}

%\subsection{Rigid fiber cross-section.}
We assume the fiber is rigid (stiffer than the matrix) and thin (the radius~$r$ is much less than the problem characteristic length).
Under geometrically exact beam theory (rigid cross-section),
%That is, we assume $r<<L$, where $r$ is the radius of the fiber cross-section, and $L$ is the fiber length.
the fiber domain~$\Omega_{F}$ is defined as
\begin{equation}\label{eq:fib:position_ref}
\Omega_{F} = \big\{ \vec{X}(\theta^{\alpha},s) = \vec{X}_c(s) + \theta^{\alpha}\vec{D}_{\alpha}(s) \big\},
% \vec{X}(\theta^{\alpha},s) = \vec{X}_c(s) + \theta^{\alpha}\vec{D}_{\alpha}(s),
\end{equation}
parametrised in terms of arclength~$s\in [0,\,L]$ along the center line~$\vec{X}_c(s)$ of the beam of length $L$.
Moreover, an orthonormal triad $[\vec{D}_1,\,\vec{D}_2,\,\vec{D}_3]$ with convective coordinates $\theta^i = (\theta^{\alpha},s)\in\tilde{\Omega}_0$ $(i=1,\,2,\,3;\,\alpha=1,\,2)$ is introduced, were $\vec{D}_{\alpha}$ span the plane cross section of the beam.
The deformation field is
\begin{equation}\label{eq:fib:position}
\tilde{\vec{x}}(\theta^{\alpha},s) = \fib{\vec{\varphi}}(s) + \theta^{\alpha}\vec{d}_{\alpha}(s).
\end{equation}
Here, the orthonormal tried $\vec{d}_i$ is related to the reference triad via the rotation tensor $\fib{\ten{R}}\in SO(3)$, i.e. $\fib{\ten{R}} = \vec{d}_i\otimes\vec{D}_i$.
Above and further, Einstein summation convention is used.
%Then, from~\eqref{eq:fib:position_ref} and \eqref{eq:fib:position}, the fiber deformation field is
%\begin{equation}\label{eq:u_fib}
%	\fib{\x}\!\left(\fib{\X}(\theta^\alpha,s)\right) = \fib{\vec{\varphi}}(s) + \fib{\ten{R}}(s)\left(\fib{\X}-\fib{\X}_c(s)\right)
%	\quad\text{ in }\Omega_{F},
%\end{equation}
%where 
%%$\ten{R}_0$ is the reference fiber orientation \rev{(it can depend on $s$)}, and 
%$\fib{\X}_c(s)$ is the coordinates of the centerline point corresponding to the arc-length~$s\in[0,L]$.
%%Without loss of generality, we assume that $\abs{\drv{\x_c}{s}}=1$.
%%By abuse of notation, in what follows. we denote $\fib{\x}(s) = \fib{\x}(\x_c(s))$.

%\begin{proof}
%	We have
%	\begin{equation}\label{eq:kin1}
%	\tilde{\vec{X}}(\theta^{\alpha},s) = \tilde{\vec{X}}_0(s) + \theta^{\alpha}\vec{D}_{\alpha}(s),
%	\end{equation}
%	and
%	\begin{equation}\label{eq:kin2}
%	\tilde{\vec{x}}(\theta^{\alpha},s) = \fib{\vec{\varphi}}(s) + \theta^{\alpha}\vec{d}_{\alpha}(s).
%	\end{equation}	
%	From~\eqref{eq:kin1}, it holds
%	\begin{align}
%		\theta^1 &= \vec{D}_{1}(s)\cdot(\tilde{\vec{X}}(\theta^{\alpha},s) - \tilde{\vec{X}}_0(s))\\
%		\theta^2 &= \vec{D}_{2}(s)\cdot(\tilde{\vec{X}}(\theta^{\alpha},s) - \tilde{\vec{X}}_0(s))\\
%		0 &=\vec{D}_{3}(s)\cdot\left(\tilde{\vec{X}}(\theta^{\alpha},s) - \tilde{\vec{X}}_0(s)\right)
%	\end{align}	
%	Substituting this to~\eqref{eq:kin2}, we obtain
%	\begin{align}
%	\fib{\x}\!\left(\fib{\X}(\theta^\alpha,s)\right) &= \fib{\vec{\varphi}}(s) + \sum_{i=1}^{3}\vec{d}_i\otimes\vec{D}_i\left(\fib{\X}-\fib{\X}_c(s)\right)\\
%	&=  \fib{\vec{\varphi}}(s) + \fib{\ten{R}}(s)\left(\fib{\X}-\fib{\X}_c(s)\right).
%	\end{align}
%	
%\end{proof}



Let us denote by $A(s)$ and $C(s)$ respectively the fiber cross-section and its boundary corresponding to the arc-length~$s$.
Moreover, it holds
\begin{equation}\label{eq:zero_integrals}
\int\limits_{A(s)}\theta^{\alpha}\vec{d}_{\alpha}(s)\d A = \int\limits_{C(s)}\theta^{\alpha}\vec{d}_{\alpha}(s)\d C = 0.
\end{equation}
The Lagrange multipliers~$\vec{\mu}$ can be decomposed as
\begin{align}\label{key}
\vec{\mu}\big|_{\Circ(s)} &= \vec{\bar{\mu}}(s) + \vec{\tilde{\mu}}(\theta^{\alpha}),
\quad\text{where}\quad
\vec{\bar{\mu}}(s) = \int\limits_{C(s)}\vec{\mu}\d C,
\quad
\int\limits_{C(s)}\vec{\tilde{\mu}}\d C = 0, \\
\vec{\mu}\big|_{\Area_{0,L}} &= \vec{\bar{\mu}}_{0,L} + \vec{\tilde{\mu}}_{0,L}(\theta^{\alpha}),
\quad\text{where}\quad
\vec{\bar{\mu}}_{0,L} = \int\limits_{\Area_{0,L}}\vec{\mu}\d A,
\quad
\int\limits_{\Area_{0,L}}\vec{\tilde{\mu}}_{0,L}\d A = 0,
\end{align}
where the average part~$\vec{\bar{\mu}}$ corresponds to the resulting force applied to the cross-section, while the zero-mean part~$\vec{\tilde{\mu}}$ contains force couples and is associated to the torque.
In what follows, due to the assumption that the fiber radius~$r$ is small, we neglect the torques, i.e. $\vct{\mu}=\vec{\bar{\mu}}$.
Then, taking in account~\eqref{eq:zero_integrals}, we have
\begin{align}\label{eq:LM_decomposition}
\int\limits_{C(s)}\fib{\x}\cdot\vec{\delta\mu}\d C
&=
\abs{C}\,\fib{\vec{\varphi}}(s)\cdot\vec{\delta\bar{\mu}}(s),
%+
%\int\limits_{C(s)}\theta^{\alpha}\vec{d}_{\alpha}\cdot\vec{\delta\tilde{\mu}}\d C, 
\\	
\int\limits_{\partial\Omega_{F,1/2}}\fib{\x}\cdot\vec{\delta\mu}\d C
&=
\abs{A}\,\fib{\vec{\varphi}}(s_{0,L})\cdot\vec{\delta\bar{\mu}}_{0,L},
%+
%\int\limits_{\partial\Omega_{F,1/2}}\theta^{\alpha}\vec{d}_{\alpha}\cdot\vec{\delta\tilde{\mu}}\d C.
\end{align}
hence,
\begin{equation}\label{eq:LAeq}
\begin{aligned}
\!\!\!\!\int\limits_{\Omega_{M}\cap\Omega_{F}} \!\!\!\!\vec{\delta\mu} \cdot(\mtx{\x}-\fib{\x})\d V
%&=
%\int\limits_{\Omega_{M}\cap\Omega_{F}} \!\!\!\!\vec{\delta\mu} \cdot\biggl(\mtx{\x}-\fib{\vec{\varphi}} - \fib{\ten{R}}\left(\X-\X_{c}\right)\biggr)\d V \\
&=
\int\limits_{\partial\Omega_{F,3}} \vec{\delta\mu} \cdot(\mtx{\x}-\fib{\x})\d V
+
\int\limits_{\partial\Omega_{F,1/2}} \vec{\delta\mu} \cdot(\mtx{\x}-\fib{\x})\d V
\\
&=
\abs{C}\!\int\limits_{0}^{L}\vec{\delta\bar{\mu}}(s) \cdot\left(\frac{1}{\abs{C}}\!\int\limits_{C(s)} \mtx{\x}\d C - \fib{\vec{\varphi}}(s)\right)\d s \\
&+
\abs{A}\!\!\sum_{s\in\{0,L\}} \vec{\delta\bar{\mu}}_{0,L} \cdot\left(\frac{1}{\abs{A}}\!\!\int\limits_{A(s)} \mtx{\x}\d A -\fib{\vec{\varphi}}(s) \right)
\end{aligned}
\end{equation}
Likewise,
\begin{equation}\label{eq:LAterm}
\int\limits_{\Omega_{M}\cap\Omega_{F}} \!\!\!\!\vec{\mu} \cdot\vec{\delta\fib{\varphi}}\d V
=
\abs{C}\!\int\limits_{0}^{L}\vec{\bar{\mu}} \cdot \vec{\delta \fib{\varphi}}\d s
+
\abs{A}\!\!\sum_{s\in\{0,L\}} \vec{\bar{\mu}}_{1,2}(s) \cdot\vec{\delta \fib{\varphi}}(s).
\end{equation}


%We also assume a thin fiber of small radius~$r$.
Let us consider a natural continuation of matrix solution inside the fiber domain~$\Omega_{F}$.
Such continuation of the solution will produce an error which depends on fiber radius~$r$, see~\cite{Koeppl2017}.
Moreover, under some regularity assumptions, we have
%\begin{equation}\label{key}
%\abs{\mtx{\x}(\theta^{\alpha},s) - \mtx{\x}(0,s)} \le C\,r,
%\end{equation}
\begin{equation}\label{eq:mean2center}
\abs{\frac{1}{\abs{C}}\!\int\limits_{C(s)} \mtx{\x}\d C - \mtx{\x}(\X_c(s))} \le C\,r.
\end{equation}
Thus, under thin fiber assumption, we will consider the reduced model with the matrix solution extended into the fiber domain, and the circumference average of the matrix deformation in the coupling condition is replaced by the matrix deformation at the fiber centerline.
%this solution~$\mtx{\x}(\X)$ admits the following expansion in the vicinity of $\mtx{\x}(\X_{c})$:
%\begin{equation}\label{key}
%\mtx{\x}(\theta^{\alpha},s) = \mtx{\x}(\X_{c}(s)) + \mtx{\ten{F}}(\X_{c}(s))\cdot\left(\theta^{\alpha}\vec{D}_{\alpha}(s)\right) + \O\left((\theta^{\alpha})^2\right),
%\end{equation}
%Then, taking in account~\eqref{eq:zero_integrals}, we have
%\begin{equation}\label{eq:red_pb:pos_cond}
%\frac{1}{\abs{C}}\!\int\limits_{C(s)} \mtx{\x}\d C = \mtx{\x}(\X_{c}) +  \O(r^2)
%\end{equation}
Under these assumptions, using~\eqref{eq:LAeq} and~\eqref{eq:LAterm}, the variational form~\eqref{eq:VariationalForm} yields
\begin{equation}\label{eq:tot_system}
\begin{aligned}
&\int\limits_{\Omega_{M}} \drv{\Psi_{M}}{\ten{F}}:\nabla\vec{\delta\mtx{x}} \d V
+
\int\limits_{\partial\Omega_{N}} \!\!\vec{t}_{ext}\cdot\vec{\delta\mtx{x}} \d S
+\\
&\hspace{10ex}+\abs{C}\!\int\limits_{0}^{L}\vec{\mu} \cdot \vec{\delta\mtx{x}}\left(\X_c(s)\right)\d s
+
\abs{A}\!\!\!\sum_{s\in\{0,L\}} \!\!\!\vec{\mu}_{0,L} \cdot\vec{\delta\mtx{x}}\left(\X_c(s)\right)
= 0, 
\\
&\int\limits_{0}^{L}\drv{\Psi_{F}}{\fib{\vec{\varphi}}^{\prime}}\cdot\vec{\delta\fib{\varphi}}^{\prime}\, \d s
-
\abs{C}\!\int\limits_{0}^{L}\vec{\mu} \cdot \vec{\delta\fib{\varphi}}\d s
-
\abs{A}\!\!\sum_{s\in\{0,L\}} \vec{\mu}_{0,L} \cdot\vec{\delta\fib{\varphi}}(s)
= 0,
\\	
&\int\limits_{0}^{L}\drv{\Psi_{F}}{\fib{\ten{R}}}:\ten{\delta\fib{R}}\, \d s
= 0, 
\\
&\int\limits_{0}^{L}\vec{\delta\mu} \cdot\left(\fib{\vec{\varphi}}(s)-\mtx{\x}(\X_c(s))\right)\d s
= 0,
\qquad 
\fib{\vec{\varphi}}(s_{0,L}) = \mtx{\x}(\X_c(s_{0,L})),
\end{aligned}
\end{equation}
for all $\vec{\delta \mtx{x}}\in\HS_{M}(\Omega_{M})$, $\vec{\delta\fib{\varphi}}\in\HS_{\vec{\fib{\varphi}}}([0,L])$, $\ten{\delta \fib{R}}\in\HS_{\ten{\fib{R}}}([0,L])$, $\vec{\delta\mu}\in\HS_{\vec{\fib{\varphi}}}^\prime([0,L])$.
%Remind that $\vec{\mu}$ and $\vct{\mu}_{1,2}$ have different units.
%completed with the constitutive laws
%\begin{align}\label{key}
%\ten{P}_{M} & = \drv{\Psi_{M}}{\nabla\mtx{\x}}\left(\nabla\mtx{\x}\right),
%&
%\vec{N} &= \drv{\Psi_{F}}{\left(\drv{\fib{\vec{\varphi}}}{s}\right)}\left(\drv{\fib{\vec{\varphi}}}{s}, \fib{\ten{R}}\right),
%&
%\ten{Q} &= \drv{\Psi_{F}}{\fib{\ten{R}}}\left(\drv{\fib{\vec{\varphi}}}{s}, \fib{\ten{R}}\right).
%\end{align}
%which are defined by the form of the free energy density in~\eqref{eq:fib:FreeEnergy}.

We consider the fiber strain energy model in the form of Simo--Reissner beam theory~\cite{Simo1985,betsch2002b,weeger2017,steinbrecher2019c}:
\begin{gather}
\tilde{\Psi}(\fib{\vec{\varphi}}^{\prime},\fib{\ten{R}}) = \frac{1}{2}\left(\vec{\eps}\cdot\stiffnessC\vec{\eps} + \frac{1}{2}\vec{\kappa}\cdot\stiffnessD\vec{\kappa}\right), \\
\vec{\eps} = \fib{\ten{R}}^T\fib{\vec{\varphi}}^{\prime}-\vec{D_3},
\qquad
\vec{\kappa}\times \vec{v} = \fib{\ten{R}}^T\fib{\ten{R}}^{\prime}\vec{v} \quad \forall\vec{v}.
\end{gather}
where $\vec{\eps}$ is known as the axial-shear strain vector, $\vec{\kappa}$ is the torsional-bending strain vector representing the curvature, $\stiffnessC = \op{Diag}[GA,\,GA,\,EA]$ and $\stiffnessD = \op{Diag}[EI_1,\,EI_2,\,GJ]$,
where $E$ is Young's modulus, $G=\frac{E}{2\,(1+\nu)}$ is shear modulus with Poisson ratio~$\nu$, $A$ is cross area, $I_j$ are second moments of area (planar), $J$ torsion constant (polar second moment), $k_j$ are shear correction factors.
%Typically $J = I_1 + I_2$ and $k_1=k_2=\frac{5}{6}$.

Any orthogonal matrix can be represented as matrix exponential of a skew-symmetric matrix, i.e. $\fib{\ten{R}} = \Exp{[\vec{\theta}]_{\times}}$, where $[\vec{\theta}]_{\times}\vec{v} = \vec{\theta}\times\vec{v}$ for all~$\vec{v}$.
Then,
\begin{align}\label{key}
\drv{\Psi_{F}}{\fib{\vec{\varphi}}^{\prime}}\cdot\vec{\delta\fib{\varphi}}^{\prime}
&=
\vec{n}\cdot\vec{\delta\fib{\varphi}}^{\prime} \\
\drv{\Psi_{F}}{\fib{\ten{R}}}:\ten{\delta\fib{R}}
&=
\drv{\Psi_{F}}{\fib{\ten{R}}}:\ten{\fib{R}}\,\left[\vec{\delta\theta}\right]_{\times}
=
\vec{m}\cdot\vec{\delta\theta}^{\prime} - \left(\fib{\vec{\varphi}}^{\prime}\times\vec{n}\right)\cdot\vec{\delta\theta}
\end{align}
where
\begin{equation}\label{eq:def_n_m}
\vec{n} = \fib{\ten{R}}\stiffnessC\left(\fib{\ten{R}}^T\fib{\vec{\varphi}}^{\prime}-\vec{D_3}\right),
\qquad
\vec{m} = \fib{\ten{R}}\stiffnessD\vec{\kappa}.
\end{equation}






Note that since we neglected the torque in the coupling, there is no additional condition for the rotation~$\fib{\ten{R}}$.
Thus, the system~\eqref{eq:tot_system} can not have a unique solution, since for any solution $(\vec{u}_{M}, \vec{r}, \ten{R}_{F})$ to~\eqref{eq:tot_system} and any rotation~$\ten{\hat{R}}$ around~$\vec{D}_3$, $(\mtx{\vec{\varphi}}, \fib{\vec{\varphi}}, \fib{\ten{R}}\ten{\hat{R}})$ is also solution to~\eqref{eq:tot_system}.

Since the effects of fiber torsion are neglected, we only have to fix fix the rotation around~$\vec{D}_3$.
The simplest way is to impose additional moment in one of the fiber ends (here at $s=L$):
\begin{equation}\label{key}
\vec{m}(L) = [0, \, 0, \, \vec{d}_1\cdot\vec{D}_2]\tp.
%\begin{bmatrix}
%\vec{d}_2\cdot\vec{d}_3 \\ 0\\ 0
%\end{bmatrix}.
\end{equation}

Thus, from~\eqref{eq:tot_system}, we eventually write the coupled
matrix/fiber system for the unknowns $\mtx{\x}\in\HS_{M}(\Omega_{M})$, $\fib{\vec{\varphi}}\in\HS_{\vec{\fib{\varphi}}}([0,L])$, $\vec{\theta}\in\HS_{\vec{\theta}}([0,L])$, $\vec{\mu}\in\HS_{\vec{\fib{\varphi}}}^\prime([0,L])$:
\begin{align}\label{eq:tot_system_final}
&\int\limits_{\Omega_{M}} \drv{\Psi_{M}}{\ten{F}}:\nabla\vec{\delta\mtx{x}} \d V
+
\int\limits_{\partial\Omega_{N}} \!\!\vec{t}_{ext}\cdot\vec{\delta\mtx{x}} \d S
+
\\
&\hspace{10ex}+\abs{C}\!\int\limits_{0}^{L}\vec{\mu} \cdot \vec{\delta\mtx{x}}\left(\X_c(s)\right)\d s
+
\abs{A}\!\!\!\sum_{s\in\{0,L\}} \!\!\!\vec{\mu}_{s} \cdot\vec{\delta\mtx{x}}\left(\X_c(s)\right)
= 0,  
\\
&\int\limits_{0}^{L}\left(\vec{n}^{\prime}
+
\abs{C}\vec{\mu}\right) \cdot \vec{\delta\fib{\varphi}}\d s
= 0,
\qquad
\vec{n}(0) = \abs{A} \vec{\mu}_{0},
\qquad
\vec{n}(L) = \abs{A} \vec{\mu}_{L},
\\	
&\int\limits_{0}^{L}\left(\vec{m}^{\prime} + \fib{\vec{\varphi}}^{\prime}\times\vec{n}\right)\cdot\vec{\delta\theta}\, \d s
= 0,
\qquad
\vec{m}(0) = \vec{0},
\qquad
\vec{m}(L) = [0, \, 0, \, \vec{d}_1\cdot\vec{D}_2]\tp,
\\
&\int\limits_{0}^{L}\vec{\delta\mu} \cdot\left(\fib{\vec{\varphi}}(s)-\mtx{\x}(\X_c(s))\right)\d s
= 0,
\qquad 
\fib{\vec{\varphi}}(s_{0,L}) = \mtx{\x}(\X_c(s_{0,L})),
\end{align}
for all $\vec{\delta \mtx{x}}\in\HS_{M}(\Omega_{M})$, $\vec{\delta\fib{\varphi}}\in\HS_{\vec{\fib{\varphi}}}([0,L])$, $\vec{\delta\theta}\in\HS_{\vec{\theta}}([0,L])$, $\vec{\delta\mu}\in\HS_{\vec{\fib{\varphi}}}^\prime([0,L])$, where $\vec{n}(\vec{\varphi}^{\prime},\fib{\ten{R}})$ and $\vec{m}(\fib{\ten{R}})$ are given by constitutive equations~\eqref{eq:def_n_m}.




\subsection{IGA discretization}

Let $\CollocSet = \{s_k, \; k=1..n\}$ be a set of $n$ points on $[0,L]$, such that $s_k\notin\{0,L\}$, and $\bar{\CollocSet} = \CollocSet\cup\{0,L\}$.
We introduce
$\TestSpace_{\CollocSet}= \vspan\{\delta(s-s_k), \; s_k\in\CollocSet\}^3,$
where $\delta(s)$ denotes Dirac $\delta$-function.
Then, for discretization of the system~\eqref{eq:tot_system_final}, we consider a Petrov-Galerkin type approximation, where $\vec{\delta\fib{\varphi}}$, $\vec{\delta\theta}$, $\vec{\delta\mu}$ and $\vec{\mu}$ are from $\TestSpace_{\CollocSet}$, $\fib{\vec{\varphi}}$ is in an appropriate spline space~$\TrialSpace_{\fib{\vec{\varphi}}}$ with knots~$\bar{\CollocSet}$, and $\fib{\ten{R}}$ is parametrized using quaternion~$\vec{q}(s)\in\R^4$, $\abs{\vec{q}(s)}=1$ ($\vct{q}$ living in an appropriate spline space~$\TrialSpace_{\vec{q}}$ with knots~$\bar{\CollocSet}$) as follows
\begin{equation}\label{key}
\fib{\ten{R}}
=
\begin{bmatrix}
q_1^2 - q_2^2 - q_3^2 + q_4^2, &
2\,(q_1\,q_2 - q_3\,q_4), &
2\,(q_1\,q_3 + q_2\,q_4),
\\
2\,(q_1\,q_2 + q_3\,q_4), &
-q_1^2 + q_2^2 - q_3^2 + q_4^2, &
2\,(q_2\,q_3 - q_1\,q_4),
\\
2\,(q_1\,q_3 - q_2\,q_4), &
2\,(q_2\,q_3 + q_1\,q_4), &		
-q_1^2 - q_2^2 + q_3^2 + q_4^2
\end{bmatrix}.
\end{equation}
We use the standard IGA approximation for the matrix material.
%Thus, for any $\vec{\mu}\in\TestSpace_{\CollocSet}$,
%\begin{equation}\label{key}
%\vec{\mu}(s) = \sum_{k=1}^{n}\vec{\lambda}_{s_k}\,\delta(s-s_k)
%\end{equation}
%where we denote 

Let us denote $\vec{\lambda}_{s_k} = \abs{C}\vec{\mu}(s_k)$, $\vec{\lambda}_{0}=\abs{A}\vec{\mu_{0}}$ and $\vec{\lambda}_{L}=\abs{A}\vec{\mu_{L}}$.
Note that $\vec{\lambda}_0$ and $\vec{\lambda}_{L}$ have units different from those of $\vec{\lambda}_{s}$, $s\in\CollocSet$.
Then, our Petrov-Galerkin approximation leads to the isogeometric collocation method discussed in~\cite{weeger2017}.
As in~\cite{weeger2017}, in order to avoid locking, we also consider $\vec{n}$ and $\vec{m}$ as additional unknowns living in appropriate spline spaces $\TrialSpace_{\vec{n}}$ and $\TrialSpace_{\vec{m}}$ respectively.
Thus, from~\eqref{eq:tot_system_final} we obtain eventually the system
\begin{align}\label{eq:IGAcolloc_system}
&\int\limits_{\Omega_{M}} \drv{\Psi_{M}}{\ten{F}}:\nabla\vec{\delta\mtx{x}} \d V
+
\int\limits_{\partial\Omega_{N}} \!\!\vec{t}_{ext}\cdot\vec{\delta\mtx{x}} \d S
+
\sum_{s\in\bar{\CollocSet}}\vec{\lambda}_{s} \cdot \vec{\delta\mtx{x}}\left(\X_c(s)\right)
= 0,  
\\
&\vec{n}^{\prime}(s)
+
\vec{\lambda}_{s}
= 0,\quad s\in\CollocSet,
\qquad
\vec{n}(0) = \vec{\lambda}_{0},
\qquad
\vec{n}(L) = \vec{\lambda}_{L},
\label{eq:fib_load_eq}
\\	
&\vec{m}^{\prime}(s) + \fib{\vec{\varphi}}^{\prime}(s)\times\vec{n}(s)
= 0,\quad s\in\CollocSet,
\quad
\vec{m}(0) = \vec{0},
\quad
\vec{m}(L) = [0, \, 0, \, \vec{d}_1(\vec{q})\cdot\vec{D}_2]\tp,
\\
&\fib{\vec{\varphi}}(s)=\mtx{\x}(\X_c(s)), \quad s\in\bar{\CollocSet}, 
\label{eq:position_coupling_eq}
\\
&\vec{n} = \fib{\ten{R}}(\vec{q})\,\stiffnessC\left(\fib{\ten{R}}\tp(\vec{q})\,\fib{\vec{\varphi}}^{\prime}-\vec{D_3}\right),
\quad
\vec{m} = \fib{\ten{R}}(\vec{q})\,\stiffnessD\vec{\kappa}(\fib{\ten{R}}(\vec{q})), 
\quad
\vec{q}\cdot\vec{q} = 1, 
\quad \text{ in }\bar{\CollocSet}.
\end{align}
Note that due to the lines~\eqref{eq:fib_load_eq} and~\eqref{eq:position_coupling_eq}, Lagrange multipliers~$\vec{\lambda}_{s}$ and the centerline deformation~$\fib{\vec{\varphi}}$ can be eliminated using a suitable discrete Null-Space reduction scheme.






\subsection{Numerical example}
TO DO


\subsection{Perspectives}

In the proposed reduced coupling model, the assumptions made lead to two kind of errors.
The first one is provided by continuation of the matrix material solution inside the fiber domain.
The second is due to replacement of the circumference average of the matrix deformation in the coupling condition by the matrix deformation at the fiber centerline.
Moreover, we also neglected the torque produced by the fiber-matrix interaction force.
Therefore, for the next step, we are going to address the following question
\begin{itemize}
	\item Estimation the error produced by the continuation of the matrix material solution inside the fiber domain, which can be done in line of~\cite{Koeppl2017}.
	\item Derivation of additional coupling condition involving the fiber-matrix interaction torque.
%	, using the higher order expansion with respect to the fiber radius~$r$ of the circumference average of the matrix deformation in the coupling condition by the matrix deformation at the fiber centerline.
\end{itemize}




==> header.tex <==
\usepackage{babel}
\usepackage{amssymb,amsmath,mathrsfs}
\usepackage{graphicx,psfrag,color,rotate}
\usepackage{tikz}

\renewcommand{\vec}{\boldsymbol}
\renewcommand{\d}[1][]{\ensuremath{\,\mathrm{d}#1}}
\renewcommand{\thefootnote}{\fnsymbol{footnote}}
\renewcommand{\arraystretch}{1.5}
\newcommand{\tc}[1]{#1}
\newcommand{\mat}{\vec}
\newcommand{\mathch}{\mathcal}
\newcommand{\indi}[1]{\ensuremath{\operatorname{#1}}}
\newcommand{\op}[1]{\ensuremath{\operatorname{#1}}}
\newcommand{\LM}{\ensuremath{\operatorname{LM}}}
\newcommand{\DIV}{\ensuremath{\operatorname{Div}}}
\newcommand{\Div}{\ensuremath{\operatorname{Div}}}
\renewcommand{\div}{\ensuremath{\operatorname{div}}}
\newcommand{\Grad}{\ensuremath{\operatorname{Grad}}}
\newcommand{\grad}{\ensuremath{\operatorname{grad}}}
\newcommand{\nablaq}[1]{\ensuremath{\nabla_{\hspace{-0.9mm}\mbox{\begin{scriptsize}$\mathrm{#1}$\end{scriptsize}}}}\hspace{0.9mm}}
\newcommand{\dnablaq}[1]{\ensuremath{\overline{\nabla}_{\hspace{-0.9mm}\mbox{\begin{scriptsize}$\mathrm{#1}$\end{scriptsize}}}}\hspace{0.9mm}}
\newcommand{\ddnablaq}[1]{\ensuremath{\overline{\overline{\nabla}}_{\hspace{-0.9mm}\mbox{\begin{scriptsize}$\mathrm{#1}$\end{scriptsize}}}}\hspace{0.9mm}}
\newcommand{\Deltaq}[1]{\ensuremath{\Delta_{\hspace{0mm}\mbox{\begin{scriptsize}$\mathrm{#1}$\end{scriptsize}}}}}
\newcommand{\setN}[1]{\ensuremath{\mathbb{#1}}}
\newcommand{\transp}{\ensuremath{^{\scriptstyle \mathrm{T}}}}
\newcommand\circlearound[1]{%
  \tikz[baseline]\node[draw,shape=circle,anchor=base] {#1} ;}
\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
\newcommand{\Cross}{\mathbin{\tikz [x=1.4ex,y=1.4ex,line width=.25ex] \draw (0.1,0.1) -- (0.9,0.9) (0.1,0.9) -- (0.9,0.1);}}
\newcommand{\punkt}[1][.]{\ensuremath{\rlap{\,{#1} }}}
\newcommand{\komma}[1][,]{\ensuremath{\rlap{\,{#1} }}}
\newcommand{\an}{{\text{e}}}
\newcommand{\s}{{\mathfrak{s}}}
\newcommand{\cross}{\vec{\times}}
\newcommand{\RR}     {\mbox{\sffamily{\bfseries R}}}
\newcommand{\KK}     {\mbox{\sffamily{\bfseries K}}}
\newcommand{\uu}     {\mbox{\sffamily{\bfseries u}}}
\newcommand{\ZERO}   {\mbox{\sffamily{\bfseries 0}}}
\newcommand{\DDelta} {\mbox{\sffamily{\bfseries $\Delta$}}} 



